eclingo: A solver for Epistemic Logic Programs

We describe eclingo, a solver for epistemic logic programs under Gelfond 1991 semantics built upon the Answer Set Programming system clingo. The input language of eclingo uses the syntax extension capabilities of clingo to define subjective literals that, as usual in epistemic logic programs, allow for checking the truth of a regular literal in all or in some of the answer sets of a program. The eclingo solving process follows a guess and check strategy. It first generates potential truth values for subjective literals and, in a second step, it checks the obtained result with respect to the cautious and brave consequences of the program. This process is implemented using the multi-shot functionalities of clingo. We have also implemented some optimisations, aiming at reducing the search space and, therefore, increasing eclingo's efficiency in some scenarios. Finally, we compare the efficiency of eclingo with two state-of-the-art solvers for epistemic logic programs on a pair of benchmark scenarios and show that eclingo generally outperforms their obtained results. Under consideration for acceptance in TPLP.

==> letter.tex <==
%!TEX root = paper.tex
\newpage
\pagestyle{empty}
\newcommand\revtext[1]{\emph{\color{blue}#1}}
We wish to thank the reviewers for their comments and suggestions that have surely helped to improve the paper. 
One major change in the paper is the removal of the optimisation technique we had called ``completion atoms'': \eclingo{} was building the associated rules but, due to a bug in the code, they were never actually added. After checking their addition, we noticed that they did not provide any significative improvement and decided to suppress them by now (updating the benchmark times accordingly), until a more exhaustive study of their effect is performed. 

We have implemented all the minor changes in the reviews. There were no suggested major changes, so we just provide below one minor clarification.

{\bf Reviewer 3}

\begin{enumerate}[label=R3.\arabic*]
\item \revtext{A minor annotation: in Section 3, if the commas in the head of the rule
\begin{align*}
    H_1,\dots,H_m  \text{ \texttt{:-} }  B_1,\dots,B_n.
\end{align*}
represent a disjunction, what do the commas in the body represent?
If they represent a conjunction of literals, a different notation should be used for the head atoms.}

We have added the following clarification: ``As happens in sequent calculus, commas in the antecedent (the body) represent a conjunction whereas commas in the consequent (the head) represent a disjunction.'' 
%
This was one recent notation change introduced in \clingo{} that is directly inherited by \eclingo{}. Still, the use of `$;$' for head disjunction is also available.
\end{enumerate}
\newpage
\pagestyle{plain}    
\setcounter{page}{1}
